Deep Neural Networks

Deep Neural Networks (DNNs) are universal function approximators providing state-of- the-art solutions on wide range of applications. Common perceptual tasks such as speech recognition, image classification, and object tracking are now commonly tackled via DNNs. Some fundamental problems remain: (1) the lack of a mathematical framework providing an explicit and interpretable input-output formula for any topology, (2) quantification of DNNs stability regarding adversarial examples (i.e. modified inputs fooling DNN predictions whilst undetectable to humans), (3) absence of generalization guarantees and controllable behaviors for ambiguous patterns, (4) leverage unlabeled data to apply DNNs to domains where expert labeling is scarce as in the medical field. Answering those points would provide theoretical perspectives for further developments based on a common ground. Furthermore, DNNs are now deployed in tremendous societal applications, pushing the need to fill this theoretical gap to ensure control, reliability, and interpretability.

==> application.tex <==
\iffalse
\section{Extensions}

\subsection{ICA}
We propose three extensions to standard ICA.
\begin{itemize}
    \item efficient convolutional ICA\cite{balle2014learning}
    \item Nonlinearity: Using $\sigma(Wx+b)$ instead of $Wx$
    \item Class dependancy
    \item Deep version
\end{itemize}
using entropy\cite{zhang2014entropy}
Even though well motivated, for full images the standard ICA penalty on the covariance of the activations is not always justified as it imposes in the limit that each image as its ont activations independant/decorrelated from all others. However for computer vision tasks, it is well known that tremendous images actually are very close from each other as it might depict the same scene/object but with a small translation/rotation a.k.a a small diffeomorphism. As a result, we first replace the uncorrelation penalty by minimizing an entropy on the distances, allowing to have similar activation for multiple inputs, yet, reaching some type of clustering via the entropy term.
Secondly, in the case of a target distance matrix, we provide a term allowing to impose it. Note that this loss somehow go against the reconstruction in practice when $Y$ are labels. Yet it forces the transform to somehow puts points closer in the feature space while being able to reconstruct.
\begin{equation}
    \mathcal{L}(X,Y;\Theta)=||X-\phi^{-1}\left(\phi(X)\right)||^2+ \alpha\mathcal{H}\left[\mathcal{D}[\phi(X)]\right]+(1-\alpha) d(\mathcal{D}[Y],\mathcal{D}[\phi(X)]) ,\alpha \in [0,1],
\end{equation}

\subsection{Tensor Wavelet Convolutional Layer}

The idea is as follows: to have global optimum, we need nonnegative weights. However if we do a renormalization by substracting the mean before application of the weights on the input $x$, then we can shift the weights without changing the output, yet, the mean substraction do not interfer with the maximization. 
In addition, if the weights of the filters is $0$ and renormalization is done then it is equivalent to having no renormalization put $0$-mean filters yet it allows to have global optimum.




In this section we derive and motivate two new layers allowing one to remove the bias used for example in a convolutional layer and thus leading to an unbiased deep network. We first build the notations and definition as well as deriving some properties to then present in the next section the results in term of template matching and the induced global property we inherit.
We thus consider the following operation done in the convolutional network
\begin{equation}
    z^{(l+1)}=W z^{(l)}+b,
\end{equation}
which we can rewrite with a per channel and per filter definition as
\begin{equation}
    z^{(l+1)}_k=\sum_{c=1}^C W^k_c z^{(l)}_c+b_k,
\end{equation}
where we remind that the matrix vector products implements the convolution.
The first layer we introduced is a standard renormalization layer that will substract the mean of the input to the input and forward this centered vector to the next layer. We denote the renormalization operation by 
\begin{equation}
    z^{(l+1)}=\mathcal{R}z^{(l)},
\end{equation}
with $\mathcal{R}z=z-\overline{z}$ where $\overline{z}$ represents the arithmetic mean of the input $z$ which can be rewritten via the linear operator
\begin{align}
    \overline{z}&=\mathcal{M}z,z \in \mathbb{R}^D\\
        &=\left[
        \begin{matrix}
        1/D & \dots & 1/D\\
         & \vdots & \\
         1/D & \dots & 1/D\\
        \end{matrix}
        \right] z.
\end{align}
which is also equivalent to the channel wise definition as
\begin{align}
    z^{(l+1)}_c=z^{(l)}_c-\frac{1}{C}\sum_{c=1}^C\mathcal{M}z^{(l)}_c.
\end{align}

This normalization thus acts on each input and substract its mean making this different from a batch normalization operation.
Note that if the following layer is a convolutional layer we have the following theorem.
\begin{theorem}
If the mean of the channel filters $\mathcal{M}W^k_c=0,\forall k,c$ then using the proposed renormalization does not change the output of the convolution.
\end{theorem}
\begin{proof}
\begin{align*}
z^{(l)}_k=&\sum_c W^k_c z^{*(l)}_c\\
=&\sum_c W^k_c (z^{(l)}_c-\mathcal{M}(z^{(l)}))\\
=&\sum_c W^k_c  z^{(l)}_c-\sum_{c=1}^Cdiag(\mathcal{M}W^{k}_c)\mathcal{M}z^{(l)}\\
=&\sum_c W^k_c  z^{(l)}_c
\end{align*}
\end{proof}
Also, a very interesting property that will be used in the next section is the invariance to shifts of the filters we now present.
\begin{theorem}
The output of $W\mathcal{R}z^{(l)}$ is invariant to shift of the weights as
\begin{equation}
    W\mathcal{R}z^{(l)}=W_a\mathcal{R}z^{(l)},\forall a \in \mathbb{R},
\end{equation}
with $W_a=W+A$ with $A(k,c,i,j)=1_{\{W(k,c,i,j)\not = 0\}}a$ which corresponds to shifting all the filters leading to the new convolution matrix $W+A$.
\end{theorem}
\begin{proof}
\begin{align*}
    z^{(l+1)}_k=&\sum_{c=1}^C \Big((W^k_c+A^k_c)  z^{*(l)}_c\Big)\\
    =&\sum_{c=1}^C \Big(W^k_c z^{*(l)}_c+A^k_c z^{*(l)}_c\Big)\\
    =&\sum_{c=1}^C W^k_c z^{*(l)}_c+\sum_{c=1}^C a \mathcal{M}z^{*(l)}_c\\
    =&\sum_{c=1}^C W^k_c z^{*(l)}_c
\end{align*}
since
\begin{align*}
    \sum_{c=1}^C a \mathcal{M}z^{*(l)}_c=&a\sum_{c=1}^C \mathcal{M}z^{*(l)}_c\\
    =&a\sum_{c=1}^C (\mathcal{M}z^{(l)}_c-\mathcal{M}z^{(l)})\\
    =&a\sum_{c=1}^C \Big(\mathcal{M}z^{(l)}_c-(\frac{1}{C}\sum_{c=1}^C\mathcal{M}z_c^{(l)})\Big)\\
    =&a(\sum_{c=1}^C \mathcal{M}z^{(l)}_c-\sum_{c=1}^C\mathcal{M}z_c^{(l)})\\
    =&0
\end{align*}
\end{proof}


The second layer we introduce which is new in its way of acting is the one that replaces the input invariant bias by 
\begin{align}
    z^{(l+1)}_k=&\mathcal{B}z^{(l)}_k\\
    =&z^{(l)}_k-\alpha_k\mathcal{M}z^{(l)},
\end{align}
thus allowing to have a per channel bias yet always based on the input. Note that while here we propose this layer, any layer introducing a bias and acting on the input leads to an unbiased deep network. In fact, it is clear that if the input is $0$, then its derivative w.r.t. $\alpha$ will be as well.
For example using $\mathcal{B}z^{(l)}_k=z^{(l)}_k-\alpha_k\max z^{(l)}$ or $\mathcal{B}z^{(l)}_k=z^{(l)}_k-\alpha_k \langle w,z^{(l)}\rangle $ all lead to unbiased networks.
We now see how the introduced operations and the removal of the bias allow to extend some properties defined earlier.





We also propose a new spline nonlinearity based on the absolute and defined via
\begin{equation}
    ABS(x;\textbf{A},\textbf{b},\Omega)=ReLU(x;\textbf{A},\textbf{b},\Omega)+ReLU(-x;\textbf{A},\textbf{b},\Omega),
\end{equation}
it is straightforward to see that this ends up being an elementwise absolute value nonlinearity with the choice of the spline regions determining the sign of the input.
We thus have
\begin{align}
    &ABS[\Big(abs_d(.;\textbf{a}_d,\textbf{b}_d,\Omega_d)\Big)_{d=1}^D](x)=\textbf{A}[x]+\textbf{b}[x],\nonumber\\
    &\textbf{A}=\{diag(v),v\in \{-1,1\}^D \},\textbf{b}=0,\nonumber \\
    &\Omega =\{\cap_{d=1}^D [W]_d,W \in \Omega_1 \times \dots \times \Omega_D]\},
\end{align}
with
\begin{align}
    &abs_d(x;\textbf{a}_d,\textbf{b}_d,\Omega_d)=\textbf{a}_d[x]+\textbf{b}_d[x],\nonumber\\
    &\textbf{a}_d=\{a_{d,1},a_{d,2}\},[a_{d,1}]_l=-1_{\{l=d\}},[a_{d,2}]_l=1_{\{l=d\}},\forall l,\textbf{b}_d=0,\nonumber \\
    &\Omega_d =\{\omega_1,\omega_2\},
    \omega_1 = \{x\in\mathbb{R}^D : [x]_d < 0\},
    \omega_2 = \{x\in\mathbb{R}^D : [x]_d \geq 0\},
\end{align}
We now present a simple example for the ABS case with $D=3,K=3$. We have according to the presented definition that the slopes of the splines are
\begin{align*}
    \textbf{A}=&\left\{
    \left[\begin{matrix}-1&0&0\\0&-1&0\\0&0&-1\end{matrix}\right],
    \left[\begin{matrix}-1&0&0\\0&-1&0\\0&0&1\end{matrix}\right],
    \left[\begin{matrix}-1&0&0\\0&1&0\\0&0&-1\end{matrix}\right],
    \left[\begin{matrix}-1&0&0\\0&1&0\\0&0&1\end{matrix}\right],
    \left[\begin{matrix}1&0&0\\0&-1&0\\0&0&-1\end{matrix}\right],\right.
    \\&
    \left. \left[\begin{matrix}1&0&0\\0&-1&0\\0&0&1\end{matrix}\right],
    \left[\begin{matrix}1&0&0\\0&1&0\\0&0&-1\end{matrix}\right],
    \left[\begin{matrix}1&0&0\\0&1&0\\0&0&1\end{matrix}\right]
    \right\},\\
    \textbf{b}=&\emptyset,\\
    \Omega=&\{\omega_1,\omega_2,\omega_3,\omega_4,\omega_5,\omega_6,\omega_7,\omega_8\},\\
    &\omega_1 = \{x \in \mathbb{R}^3:[x]_1< 0,[x]_2<0,[x]_3<0\},\\
    &\omega_2 = \{x \in \mathbb{R}^3:[x]_1< 0,[x]_2<0,[x]_3\geq 0\},\\
    &\omega_3 = \{x \in \mathbb{R}^3:[x]_1< 0,[x]_2\geq 0,[x]_3<0\},\\
    &\omega_4 = \{x \in \mathbb{R}^3:[x]_1< 0,[x]_2\geq 0,[x]_3\geq 0\},\\
    &\omega_5 = \{x \in \mathbb{R}^3:[x]_1\geq 0,[x]_2<0,[x]_3<0\},\\
    &\omega_6 = \{x \in \mathbb{R}^3:[x]_1\geq 0,[x]_2<0,[x]_3\geq 0\},\\
    &\omega_7 = \{x \in \mathbb{R}^3:[x]_1\geq 0,[x]_2\geq 0,[x]_3<0\},\\
    &\omega_8 = \{x \in \mathbb{R}^3:[x]_1\geq 0,[x]_2\geq 0,[x]_3\geq 0\},
\end{align*}
and we thus have when given some inputs that
\begin{align*}
    ABS([1,2,3]^T,\textbf{A},\textbf{b},\Omega)&=A_8[1,2,3]^T\\
                                            &=[1,2,3]^T,\\
    ABS([1,-2,3]^T,\textbf{A},\textbf{b},\Omega)&=A_6[1,-2,3]^T\\
                                            &=[1,2,3]^T,\\
    ABS([-1,-2,-3]^T,\textbf{A},\textbf{b},\Omega)&=A_1[-1,-2,-3]^T\\
                                            &=[1,2,3]^T.\\
\end{align*}
One can see that as the exact position of all the signs is determined by which $A_i$ has been selected, we have the following property
\begin{prop}
In the case of the use of ABS we have that
\begin{equation}
    \textbf{A}[x]^T\textbf{A}[x]x=x,
\end{equation}
since by definition we have that that all $A_i$ is an orthonormal matrix, $\forall i$ thus
\begin{equation}
    \textbf{A}[x]^T\textbf{A}[x]=I_D,\forall x \in \mathbb{R}^D.
\end{equation}
\end{prop}



\begin{prop}
In the case of using ABS, we now have the selection of the spline equivalent to
\[
\textbf{A}[x] = \argmax_{A_i \in \textbf{A}} || A_ix ||^2_p,p\in \mathbb{N},\forall x \in \mathbb{R}^D.
\]
\end{prop}
Note that this is different that for the case of increasing activation functions s.a. ReLU or LReLU which tried to maximized the sum of the output as opposed to the norm here.














\begin{theorem}
Given an training input data pair $(x_i, y_i=q)$ (i.e., from class $q$), the output vector $v(m)$ of a CNN (suitably trained, etc.) approximates a matched filter bank (as introduced in the intro):
%
\begin{align}
v(m) ~=~ \langle x, \tau_m \rangle
\end{align}

where $\tau_q \approx x$ and $\tau_m \perp \tau_q, m\neq q$.
\end{theorem}


In words, the CNN learns to compute a GLRT type classifier from training data, which is optimal.  
Of course this is just for the training data.




MORE ON MF.
Comment on the channel that yields 1 in the 1-hot representation (the correct class).
Comment on the other channels that yield 0 in the 1-hot rep (the incorrect classes).


FIGURE on what the MF looks like when $\bx$ is input (blurry car, etc.).

\subsection{Unbiased Deep Network}
Has we have seen in the previous sections, a deep network can be seen as a factorized affine spline. However as it was demonstrated in the secion [REF SECTION] the bias can be detrimental during learning and to obtain good generalization.
On the other hand, having no bias is not synonym o no bias inside the network. It simply means that the bias is a function of the input. As a result, e now analyze this special case as an unbiased deep neural netwok.


\section{Experiments}
\subsection{Behaviors of the template through depth}
\subsection{From activation graph to matched filter}

\richb{There is a 1-1 relationship between the activation graph (plus values) and the matched filter template.}

\richb{richb to add perceptron to this as well}

Consider the 2-layer CNN from above. 
Given a signal $x$, we can compute the output $z^2$ (suppress the superscript for now); key point is that the we can condition all of the convolution matrices based on the AT and zero out the entries that are not activated, i.e., generic $\bC$ becomes $\bC(x)$.
Thus, can compute
\begin{align}
    \bz|\bx ~=~ \bC^2(x)\bC^1(x)\bx + \bC^2(x)\bb^1 + \bb^2.
    \label{eq:z|x}
\end{align}
Now compute the $r$-th element of the output 
\begin{align}
    [\bz|\bx]_r ~&=~ [\bC^2(x)\bC^1(x)]_{r,\cdot}\bx + [\bC^2(x)\bb^1 + \bb^2]_r \nolabel \\[2mm]
    &=~ \langle [\bC^2(x)\bC^1(x)]_{r,\cdot}, \bx \rangle + [\bC^2(x)\bb^1 + \bb^2]_r.
    \label{eq:condOutput}
\end{align}
Hence, we see that the output is the inner product of the signal with a template that is the $r$-th row of the matrix $\bC^2(x)\bC^1(x)$.
\richb{what to say about the bias?  Explain why it is there:  1) it encodes priors (see DRMM), 2) it corrects for ReLU (randall to explain)}\randall{The bias is more here so that the average of the output is around 0, if the bias is removed the accuracy is not so much below especially if setting averages to 0 by hand after each convolution. Also in the case of gated activation there is no bias and they are state of the art.}
\richb{add figures from Slack}

\begin{figure}[t!]
    \centering
    \includegraphics[width=6.5in]{Figs/before_learning_test.png}
    \caption{Before Learning Templates}
    \label{fig:acttree}
\end{figure}

\begin{figure}[t!]
    \centering
    \includegraphics[width=6.5in]{Figs/before_learning_test.png}
    \caption{After Learning Templates}
    \label{fig:acttree}
\end{figure}

\begin{figure}[t!]
    \centering
    \includegraphics[width=6.5in]{Figs/experiment.png}
    \caption{Some more experimental Templates after Learning}
    \label{fig:acttree}
\end{figure}
\begin{theorem}
In a CNN (+MLP) trained for classification, given a signal $x$ from class $q$ of the training set, then 
$[\bC^2(x)\bC^1(x)]_{q,\cdot} \approx \bx^T$.
With $\bx$ contaminated by WGN, this is an approximately optimal detection statistic.
\end{theorem}

\begin{cor}
In a CNN (+MLP) trained for classification, given a signal $x$ {\em not} from class $q$ of the training set, then 
$[\bC^2(x)\bC^1(x)]_{q,\cdot} {\rm ~is~approx~orthogonal~to~} \bx^T$.
In other words, (\ref{eq:condOutput}) $\approx 0$.
\richb{will think of some notation or just say it in words.}
\end{cor}

Note: We can add in the last 2 MLP layers into all this, since the output $\bv$ can be written as 
\begin{align}
    \bv ~=~ \So\bD^2 \P \T \Big( \bD^1 \bz + \bb^1 \Big).
\end{align}


\fi

==> cutstuff.tex <==

\section{CUT STUFF that might be useful later}



We call the application of each $f^\ell$ a {\em layer} of the network.
The first operation in a given layer forms a linear combination of the entries of $x$ via a set of weights $w_{i'i,j'j,k'k}$
\begin{align}
(\C x)(i',j',k') ~=~ \sum_{k=1}^K\sum_{i=1}^{I}\sum_{j=1}^{J} w_{i'i,j'j,kk'} \, x(i,j,k) 
\label{eq:fullyCon}
\end{align}
\randall{
\begin{align}
(\C x)(i,j,k) ~=~ \sum_{k=1}^K\sum_{i'=1}^{I'}\sum_{j'=1}^{J'} w_{I'-i',J'-j',k} \, x(i+i',j+j',k) 
\label{eq:fullyCon}
\end{align}}

to create an output of size $I',J',K'$.
\richb{make sure this formula is correct on $k',k$}
Here, each entry of the input $x$ contributes to each entry of the output $\C x$ and so we call this a {\em fully connected} linear combination.
\richb{or is it in fully connected that ``each pixel entry of the input $x$ contributes to each entry of the output $\C x$ and then we average over the channels'' like in a conv layer?}\randall{You can see a fully connected (MLP) as a CNN with filters with same size as the input size and  (as opposed to smaller for CNN) and as many filters as you want output neurons}
We can write (\ref{eq:fullyCon}) more succinctly using matrix notation by vectorizing the signal $x$ across its three dimensions into the vector $\bx$ (see Figure \ref{fig:reshape}) and stacking the weights into the matrices $W^k$
\begin{align}
\C \bx ~=~ \sum_{k=1}^K W^k \bx
\label{eq:fullyConMatrix}
\end{align}
\richb{i need help writing this out for fully connected.  We can basically pull the vectorization from the ``linearization'' section into here.  we should do this because the vector representation is already known and we'll just build on it. I think the equation is the fully connected version of (\ref{eq:bigMatrix1}).}\randall{exactly, with the vectorization of the input then the MLP becomes a simple matrix vector product, the weights are in a matrix with number of rows = number of output nodes and number of columns = size of the flattened input}




Since the number of weights in (\ref{eq:fullyCon}) is enormous, it is common to simplify the general linear combination to a {\em convolution}
\begin{align}
(\C x)(i',j',k') ~=~ \sum_{k=1}^K\sum_{i=1}^{I}\sum_{j=1}^{J} w_{i'-i,j'-j,k'k} \, x(i,j,k) 
\label{eq:conv}
\end{align}
\richb{randall to figure out whether to use + or - in the conv}\randall{should be minus or it is correlation, just to follow conventions...}
Now the weights play the role of impulses responses of filters that are scanned across each channel of the image; the filter outputs are combined by averaging across all input channels.
Without loss of generality, we will ignore the details relating to boundary effects in the convolution above and assume that $I'=I$ and $J'=J$; these are typically handled by zero padding the images or boundary reflection.
The output image size can be reduced by striding the convolution, i.e., shifting the filter by multiple samples in each spatial direction.
Just as above, we can 

%-----------------



\bigskip

Convolutional Neural Networks (CNN) are a specific kind of Artificial Neural Network (ANN) topology acting on $3$-dimensional volumes of arbitrary dimensions and on which convolutions are applied implying the ability to manage those high-dimensional blocks with a reasonable amount of free parameters due to the weight sharing across positions.
On this volume $x$ of shape $(K,I,J)$ where $k$ is the depth and $(i,j)$ the usually spatial coordinate, a convolution with another $3$-dimensional volume $W$ of shape $(K,I',J')$ with $I'\leq I$ and $J' \leq J$  is defined as the linear operator $\mathcal{R}$ with
\begin{align}
    \mathcal{R}_{W}&[x](m,n)=\sum_{k=1}^K\sum_{i=1}^{I'}\sum_{j=1}^{J'}x_{k,m+i,n+j}W_{k,I'-i,J'-j},\nonumber \\
    &\forall (m,n) \in\{1,...,I-I'+1\} \times\{1,...,J-J'+1\},
\end{align}
which is equivalent to summing all the $K$ $2$-dimensional convolutions as
\begin{align}
    \mathcal{R}_{W}&[x](m,n)=\sum_{k=1}^K(x_{k,.,.}\star W_{k,.,.})(m,n),\nonumber \\
    &\forall (m,n) \in\{1,...,I-I'+1\} \times\{1,...,J-J'+1\}.,
\end{align}
where $\star$ defines the discrete convolution operator.


\begin{figure}[t!]
    \centering
    \includegraphics[width=5in]{Figs/volume.jpg}
    \caption{Depiction of one CNN layer taking the input $\out^l$ and first performing the multiple $3D$ convolutions for different filters and stacking the results to create a new volume ($1)$) followed by the application of a nonlinearity here a ReLU ($2)$) leading to the new output $\out^{l+1}$ which will become the input of a next layer.}
    \label{fig:my_label1_volume}
\end{figure}



An illustration of the operation is presented in Fig. \ref{fig:my_label1_volume}. The volume $W$ represents a filter and thus each CNN layer includes a collection of filters arranged in a filter-bank denoted as $\mathcal{W}=\{W^{(f)},f=1,...,F\}$ and for which case the complete output of the layer is a volume of shape $(I-I'+1,J-J'+1,F)$ s.t.
\begin{align}
    &\out_{m,n,f}=\mathcal{R}_{W^{(f)}}[x](m,n)+b_f,
\end{align}
where $b_f$ is a bias scalar added for each filter. Note that if all the filters in a filter-bank are of same shape, the one can see $\mathcal{W}$ as a $4$-dimension tensor with shape $(F,K,I',J')$
Note that we only present the case where convolutions are done on the valid support of both the input $x$ and the filter $W$ and without boundary conditions, generalizing the presented notations is straightforward for all the other cases.
Following this convolutional operations a pooling operation $\mathcal{P}$ and an element-wise nonlinearity $\mathcal{T}$ is applied. The order matters unless the two operations are commutative as is the case with max-pooling or mean-pooling and any monotonic function s.a. the Rectifier Linear Units (ReLU), sigmoid, hyperbolic tangent and many others. Depending on the task at hand, one can stack multiple convolutional layers to build a hierarchical representation and finally add a multilayer perceptron depending on the objective.


Since all the involved operations and functions are differentiable almost everywhere, one can use gradient descent to fit all the filter-banks $\mathcal{W}^l$ for each layer $l\in\{1,...,L\}$ and any other free parameters to minimize a user defined loss function w.r.t. a given dataset. This process is referred as backpropagation since the use of the chain rule to update the inner network parameters ends up being a backward flow of information from the last output layer. We will now present the main analysis from the paper through a conditioning of the layer w.r.t. to a given input in order to linearize it.



==> execsum.tex <==
\centerline{\Large\bf Executive Summary (Short Paper)}
\bigskip

%------------------------------------------------
\section{Introduction [1/2 page]}
%\label{sec:intro}

\paragraph{Intro to deep nets, their ascendency, and their mysteriousness}

\paragraph{Previous attempts to build a rigorous mathematical framework around deep nets}

DRMM (as a hierarchical Gaussian mixture model), 
Scattering, Soatto, etc.

\paragraph{In this paper, we build a rigorous bridge between deep nets, approximation theory, and splines}

\paragraph{In particular, we demonstrate that \dots}

Overview key contributions

\paragraph{Organization of paper}


%------------------------------------------------
\section{Background on Deep Neural Networks [1 page]}

Explain convolution, nonlinearity, pooling with focus on ReLU and softmax nonlinearities for concreteness.  Point to appendix for other nonlinearities (leaky ReLU, sigmoid, etc.)

Architectures: focus on standard convnet for concreteness, but point to appendix for discussion of other architectures like skip connections, resnet, RNN, etc.

Inference, focus on classification for concreteness

Learning via cross-entropy


%------------------------------------------------
\section{Background on Splines and Spline Operators [1 page]}

\subsection{Splines}

What is approximation theory?
Function class, parameterized approximant, error measure, optimization.
Ex: splines

\subsection{Spline Operators}

Simply vectorized spline

\subsection{Adaptive Partitioning Splines}

Boyd/Dunson stuff.



%------------------------------------------------
\section{Deep Neural Networks are Spline Operators [1 page]}

\paragraph{Theorem:}  
Standard convnet, resnet, skip connection net, and RNN with conv, ReLU, max-pool are all equivalent to a linear spline operator.

\paragraph{Remark:} Special case: ReLu/max-pooling neural nets are adaptive partitioning splines

\paragraph{Theorem:} 
The networks in the theorem above with higher-order nonlineariries like sigmoid, arctan, etc. can be approximated arbitrary closely by a linear spline operator.


%------------------------------------------------
\section{Deep Neural Network Learning as Spline Operator Approximation}

Now that we have a parameterized approximant (DNN=LSO), we can learn its parameters by optimizing a cost function that measures the deviation between the approximant and a target function/operator from some function class.

Continuing with classification inference, we pose the following approximation problem.
{\em Target} operator maps the input $X$ from class $Y$ to the output $Z = +1$ for the correct class and $Z=-1$ for all the incorrect classes.
Such a $Z$, when input into the final softmax, produces a 1-hot representation pointing to the correct class. \richb{why $\pm 1$ and not $\pm c$ or $\pm \infty$?}

{\em Error measure} is cross-entropy \richb{but cross-entropy is measured at $Y$ and not $Z$, right?}
Justify reasonableness of cross-entropy.

Thus, the approximation problem can be written as:
\[
{\sf approx~problem~softmax}
\]







%------------------------------------------------
\section{}


%------------------------------------------------
\section{}






\paragraph{}

\paragraph{}

\paragraph{}

\paragraph{}

\paragraph{}

\paragraph{}

\paragraph{}

\paragraph{}

\paragraph{}

\paragraph{}

\paragraph{}

\paragraph{}

\paragraph{}

\paragraph{}

\paragraph{The stuff below will turn into Appendices}



==> improve.tex <==
\section{Improve}

\iffalse
\subsection{Augmented Neural Networks}
In this subsection we present the augmented CNN which consist of a neural network with a last layer containing more output neurons than needed for the task at hand. This idea is not new and for example in \cite{reed2014learning,mathieu2016disentangling} autoencoders are trained with distinct neurons for different types of latent variables disentanglement.
. Combining bothproduced styloe transfer with a way to maintain a class while inteprolation on the other latent variables. We propose here the same scheme and show resultsfor CNNs. This will be particularly usefull for reconstruction tasks.
The last layer contains features for classification and reconstruction to allow full disentanglement and better path schemes.
\begin{figure}[t!]
    \centering
    \includegraphics[width=5in]{Figs/augmented.jpg}
    \caption{Augmented ANN architecture for the last layer where the first part of the neurons is used with a softmax for classification purposes while the other part is used to encode and keep track of latent variable for better overall reconstruction. The classification only uses the softmax output whereas the reconstruction uses all the output neurons, the softmax output for the class determination and the others ones for the distortions.}
    \label{augmented_loss}
\end{figure}
The output now is different and illustrated in Fig. \ref{augmented_loss}, softmax for the first part of the ANN on which classification cross-entropy and unsupervised entropy will be computed and a linear part that is only used for reconstruction and thus on which no entropy loss is applied.
\begin{figure}[t!]
    \centering
    \includegraphics[width=5in]{Figs/experiment_augmented_hybrid_loss.jpg}
    \caption{Augmented output perceptron loss on MNIST for hybrid training of reconstruction and classification. It is interesting to see that the training error decreases proportionally faster with the number of added output neurons, yet on the classification accuracy for the test set, only a more stable result is showed without increases in convergence.}
    \label{augmented_loss}
\end{figure}
In Fig. \ref{augmented_loss} one can see that the proposed augmented CNN strategy when training on MNISt with hybrid loss is able to converge on the training set faster as one augments the number of added output neurons. Yet it is not clear on the classification accuracy what are the gains. In fact, the loss gain in the training error is partly due to the fact that the network is able to reconstruct better with those added neurons, but there is not impact on the classification accuracy as they are not considered for that in the output layer.
\begin{figure}[t!]
    \centering
    \includegraphics[width=5in]{Figs/experiment_augmented_hybrid_reconstruction.jpg}
    \caption{Reconstruction examples form the trained network of Fig. \ref{augmented_loss} showing clearly that the reconstruction is better as the number of output neurons grows. The number of added neurons is written in the title per row of the subplots.}
    \label{augmented_reconstruction}
\end{figure}


\fi




\subsection{Network Inversion: Beneficial Reconstruction}
As studied in the previous section, one of the aspect of the unpredictable nature of the output of the deepnet comes from its mapping which is a many-to-one with the ''many'' being outrageously too large in general. In fact, if the system is applied on natural images, it is natural to not expect this ''many'' to map anything if given a nonnatural image, or at least, not with high confidence.
One way to limit this as well as to enforce that overfitting is done in a beneficial way, one can impose the network to construct the input. 
In fact, we have that 
\begin{align}
    &\forall x \in \text{ training set}, \exists (\alpha'_1,\dots,\alpha'_{\ell-1}) \in (\bm{\alpha^{(1)}},\dots,\bm{\alpha^{(\ell-1)}}) \text{ such that}\\
    &x \approx \mathcal{F}[(\textbf{A}^{(l)},\textbf{b}^{(l)},\alpha^{(l)})_{l=1}^{\ell-1}](z^{(\ell-1)}),\text{ for some } z^{(\ell-1)} \in \omega^{(\ell)}_{\alpha^{(\ell)}},
\end{align}
and thus if the training set is large enough given the number of possible output regions, one can hope to regularize the network by constraining its spanning possibilities in the input space, and this can even further be constraint by imposing that the final region in which $z^{(\ell)}$ belongs to is the one determining the output class, for example, if a ReLU is applied, then the region of class $k$ is defined as the one with mask with $0$ everywhere but in the $k^{th}$ dimension.

It is clear that $\mathcal{F}[(\textbf{A}^{(l)},\textbf{b}^{(l)},\alpha^{(l)})_{l=1}^{\ell-1}](z^{(\ell-1)})$ is the considered version of the inverse of the deep neural network. We now present a few results concerning this formula especially in the case of the standard use of ReLU


\subsection{Parametric Filters}
when people try to learn for example the coefficient of the ReLU after a CNN it is equivalent to finding a multiple of the filter at this exact position and channel.

which in turn is equivalent to learn an elementwise scalar multiplication with a mask.
Similarly to learn a convex activation function easily it is enough to learn multiple such mask and pool over them. This usually leads to lots of overhead and a priori having position dependent behavior is not justified in the context of convolutional neural networks as by definition convolutions is used as the input is assumed to be translation invariant.
Since stochastic gradient desent is applied on each scalar parameter ''independantly''from the others, trying to make the filters as sturctured and scalar independnat is a way to counter this drawback.
One way to do this is to learn instead of the raw filter a multiscale expension of the filter, as it is now possible to ''drastrically'' change the shape of the filter just by changing a few coefficients. For exmaple if the filters needs to be the same but with a translated mean, gradient descent will have a hard time as moving all the coefficent from the same amount is almost impossible in practice.
As a reuslt we rewrite the filters in the 




==> linear.tex <==


\iffalse
\subsection{Linearization of CNNs}

\richb{RB said this is false?  we only deal with the first convo layers of the CNN; the subsequent layers are only an old school NN -- we turn to them layer}


The CNN function $f(\bx)$ from (\ref{eq:genNN}) is a ``complicated'' nonlinear function and not immediately interpretable.
There are standard methods to deal with nonlinear functions; the idea is to a local approximation to the function that holds around a point $x_0$.
One is to compute a Taylor series and look at low-order terms (e.g., linearization); for example, if $f(\bx)$ is smooth around $\bx_0$, then a linear (affine) approximation would be
%
\begin{align}
f(\bx|\bx_0) ~\approx~ A \bx + \bd
\label{eq:linear1}
\end{align}\randall{can we use $A_{x_0}\bx + \bd_{x_0}$ ?}
%
for $\bx$ in a suitably small neighborhood around $\bx_0$ \randall{for CNN and ANN in general this does not necessarily mean that $||x-x_0||<\epsilon$ but it means that $x$ and $x_0$ implies the same activation maps and paths (position for max pooling and ReLU)}.
The matrix $A$ and offset $\bd$ provide insight into the behavior of $f$ for signals of this type.
%Another is chaos theory (how?).
%Another is splies (how - and ties into below).


The problem with the above approach is that CNNs are {\em not} smooth.
Explain and \cite{X}\randall{as any layer including CNN can be seen as a sum of affine transformation, sum over all the possible activations and when given an input, one of the component (only one) is selected and used}.
And so Taylor series cannot be applied to linearize \randall{as the complexity comes from the mixture not the functions of each mixture too}.


Nevertheless, because of the special structure of a CNN, we can find a result like (\ref{eq:linear1}) that holds without a smoothness assumption.
Moreover, we can find a closed-form formula for the matrix $A$ and offset $\bd$.  
The key is \richb{what? the ReLU and max pool structure?}\randall{the forward pass which determines which of the path/mixture are activated thus reducing the whole model to only an affine transformation which is done easily via max pooling and relu which are just indicator functions placed}


We are going to show the following: For the first 1/2 of a CNN, etc. etc. as described in (x)--(y) with ReLu and Max Pool, for a training data point $\bx_0$, we have 
\begin{align}
f(\bx_0|\bx_0) ~\approx~ A \bx_0 + \bd
\label{eq:linear2}
\end{align}


Let consider a 2-layer CNN since deeper network can be derived by recursive application of the presented analysis. We introduce the following notations for the output of respectively the first CNN layer at all position but index $k$ since it is a $3$D tensor as
\begin{equation}
    \out^1_k[x]=\mathcal{P}\Big[\mathcal{T}\Big( \mathcal{R}_{W^{(1,k)}}[x] +b^1_k\Big)\Big]
\end{equation}
where $x$ stands for the input image and $W^{(1,k)}$ the $k^{th}$ filter of the first filter-bank $\mathcal{W}^{(1)}$, $\mathcal{T}^1$ is the nonlinearity of the first layer which in our case will be a ReLU and finally $\mathcal{P}^1$ is the pooling/downsampling operation of the first layer.
For the second layer we have
\begin{equation}
    \out^2_k[\out^1[x]]=\mathcal{P}^2\Big[\mathcal{T}^2\Big( \mathcal{R}_{W^{(2,k)}}[\out^1[x]] +b^2_k\Big)\Big]
\end{equation}

We now present the input conditioning for each of the two nonlinear operators $\mathcal{T}$ and $\mathcal{P}$. Given any input $z$, we can through a forward pass observe the activations and thus w.r.t. this input, we can now see the operators as linear. For simplicity we will consider the case with max-pooling and ReLU activation. We denote this conditioning as
\begin{align}
    \mathcal{P}[x|z]:=\mathcal{P}_{z}x,\\
    \mathcal{T}[x|z]:=\mathcal{T}_{z}x,
\end{align}
where one can rewrite the operation has a product matrix vector if the inputs are reshaped accordingly. In the case where $z=x$ this is simply the result of passing an input and holding the induced states or position of the indicator functions.

We now rewrite the presented formula in matrix notation for simplification of the following derivations. We can indeed rewrite the discrete convolution through a vectorized version of the image $x$ and reshaping the filters as well. We thus end up with
\begin{align}
    \out^1[x]   &= \mathcal{P}^{1}\Bigg[\mathcal{T}^{1}\Big[W^{1} x+b^1\Big] \Bigg],\nonumber \\
    \out^1[x|x] &= \mathcal{P}^{1}_{x''}\mathcal{T}^{1}_{x'}\Big(W^{1} x+b^1\Big)
\end{align}
where $b^1$ is a vertical concatenation of all the bias repeated $n$ times to be applied on the correspond part of the corresponding filter. We thus have once conditioned on an input a linear mapping where the conditioning is denoted as
\begin{align}
    x'=&W^{1} x+b^1,\\
    x''=& \mathcal{T}^1_{x'} \Big(W^{1} x+b^1\Big).
\end{align}

For the second layer we similarly have
\begin{align}
\out^2[\out^1[x]|x]=& \mathcal{P}^{2}\Bigg[\mathcal{T}^{2}\Big[W^2 \out^{1}[x|x]+b^2\Big] \Bigg]\\
=&\mathcal{P}^{2}\Bigg[\mathcal{T}^{2}\Big[W^2  \Bigg(\mathcal{P}^{1}_{x''}  \mathcal{T}^{1}_{x'}  \Big(W^1  x+b^1\Big)\Bigg)+b^2\Big] \Bigg] \nonumber \\
=&\mathcal{P}^2_{x''''}\mathcal{T}^2_{x'''}W^2 \mathcal{P}^1_{x''}\mathcal{T}^1_{x'}W^1x\nonumber\\
&+\mathcal{P}^2_{x''''}\mathcal{T}^2_{x'''}\Big(W^2D^1_{x''}M^1_{x'}B^1+B^2\Big)\nonumber \\
=&\textbf{W}_xx+\textbf{b}_x
\end{align}
with 
\begin{align}
    x'''=&W^2  \Bigg(\mathcal{P}^{1}_{x''}  \mathcal{T}^{1}_{x'}  \Big(W^1  x+b^1\Big)\Bigg)+b^2\\
    x''''=&\mathcal{T}^{2}_{x'''}\times\Big[W^2  \Bigg(\mathcal{P}^{1}_{x''}  \mathcal{T}^{1}_{x'}  \Big(W^1  x+b^1\Big)\Bigg)+b^2\Big]\\
    \textbf{W}_x=&\mathcal{P}^2_{x''''}\mathcal{T}^2_{x'''}W^2\mathcal{P}^1_{x''}\mathcal{T}^1_{x'}W^1\\
    \textbf{b}_x=&\mathcal{P}^2_{x''''}\mathcal{T}^2_{x'''}\Big(W^2\mathcal{P}^1_{x''}\mathcal{T}^1_{x'}b^1+b^2\Big)
\end{align}
we can see that we go from two layer non linear CNN to a one layer linear CNN.
For the special case with linear activation and no max pooling we have $\mathcal{T}=I$ and $\mathcal{P}=I$ thus we can rewrite
\begin{align}
\out^2[\out^1[x]|x]=&\out^2[\out^1[x]] \nonumber \\
=&W^2W^1x+W^2b^1+b^2\nonumber
\end{align}
which is exactly the definition of a one layer linear CNN but this time without the need to be conditioned on a specific input meaning that there is no adaptivity to the input.
In fact, it is well known that a linear deep CNN is mathematically equivalent to a shallow CNN yet in practice with a better prior on the filters since they are factorized which helps during learning.
The standard nonlinear CNN framework thus allows the pooling and nonlinearity matrix to be dynamically generated for each different input. Yet, once given an input, a forward pass determines all those matrices making the whole network linear and deterministic conditioned on the activations induced by a specific input.
Concerning the shape of the matrices, we have that $W^1$ is of shape $(F^{(1)}\times P,N\times ch)$ where $ch$ is the number of channels of the inputs image, $N$ is the product of the spatial sizes $I \times J$ (thus $N
\times ch$ is the size of the flattened input). $F^{(1)}$ is the number of filters in the first filter-bank $\mathcal{W}^{(1)}$ and $P$ the number of position to be applied thus in our case $(I-I'+1)(J-J'+1)$, This generalizes for all the $W$. The matrices for the nonlnearities $\mathcal{T}_x$ are diagonal with $1$ or $0$, and the pooling matrices $\mathcal{P}_x$ are rectangular with shape $(N/s,N)$ where $N$ was the size of the right hand matrix and $s$ the support for the pooling assuming no overlapping is used. 
We now see that the dimension of $\textbf{W}_x$ is a matrix of shape $(S,N*ch)$ where $S\leq F^{(L)}$ is the number of filters in the last filter-bank times the number of positions for each of them. In the case where the CNN is deep enough to have a final template of spatial shape equal to the one of the input then  $S= F^{(L)}$, $N*ch$ represent the input image size flatten and $ch$ the number of channel, in fact the image is first flatten according to the scheme presented in Fig. \ref{x_reshaping} which is the standard technique.

We present below the shape of $W_x$ for the general case with multiple positions we denote by $p_{i}$ with $i\in \{1,...,P\}$
\begin{equation}
    \textbf{W}_x = \left( \begin{matrix}
    \textbf{W}_{x,1,p_1}^T\\
    \textbf{W}_{x,1,p_2}^T\\
    \vdots \\
    \textbf{W}_{x,1,p_P}^T\\
    \vdots\\
    \textbf{W}_{x,F^{(L)},p_1}^T\\
    \textbf{W}_{x,F^{(L)},p_2}^T\\
    \vdots \\
    \textbf{W}_{x,F^{(L)},p_P}^T\\
    \end{matrix}\right),\;\;\textbf{W}^{full}_x = \left( \begin{matrix}
    \textbf{W}_{x,1}^T\\
    \textbf{W}_{x,2}^T\\
    \vdots\\
    \textbf{W}_{x,F^{(L)}}^T\\
    \end{matrix}\right)
    \label{eq:bigMatrix1}
\end{equation}
where now each $\textbf{W}_{x,f}, \forall f \in \{1,...,F^{(L)}\}$ is a vector of same length as the flattened input $x$. For the case where the CNN template has same spatial size then we end up with $\textbf{W}^{full}_x$.
Similarly for the bias vector, it has the same length as the number of rows in $\textbf{W}_x$ and thus also depends on the number of position per filter are to be applied, in fact we have
\begin{equation}
    \textbf{b}_x = \left( \begin{matrix}
    \textbf{b}_{x,1,p_1}^T\\
    \textbf{b}_{x,1,p_2}^T\\
    \vdots \\
    \textbf{b}_{x,1,p_P}^T\\
    \vdots\\
    \textbf{b}_{x,F^{(L)},p_1}^T\\
    \textbf{b}_{x,F^{(L)},p_2}^T\\
    \vdots \\
    \textbf{b}_{x,F^{(L)},p_P}^T\\
    \end{matrix}\right),\;\;\textbf{b}^{full}_x = \left( \begin{matrix}
    \textbf{b}_{x,1}^T\\
    \textbf{b}_{x,2}^T\\
    \vdots\\
    \textbf{b}_{x,F^{(L)}}^T\\
    \end{matrix}\right)
\end{equation}

We now briefly describe the same type of notation for the case of a Multi Layer Peceptron (MLP) in order to have unified notations for a general case network. Note that a CNN with filters of spatial size $(1,1)$ is equivalent to a perceptron if the last layer had no position index and is equivalent of a perceptron with local weight sharing otherwise.
We rewrite similarly the output of a 2-layer MLP as the generalization is straightforward
\begin{equation}
    \out=\mathcal{T}^2\Bigg[W^2\mathcal{T}^1\Big[W^1x+b^1\Big]+b^2\Bigg]
\end{equation}
where one usually uses a Softmax activation operator for $\mathcal{T}^2$. For simplification we define the following operator 
\begin{equation}
    \mathcal{T}^2[x](y)=\frac{sgn(x(y))*x(y)}{\sum_{y'}sgn(x(y))*x(y)},
\end{equation}
we thus still have $\mathcal{T}^2[x](y) \in [0,1]$ and $\sum_y \mathcal{T}^2[x](y) =1$ and thus can be used to represent $p(Y=y|X=x)$. In this case, we can rewrite the operator as a deterministic diagonal matrix multiplication once conditioned on an input which lead to the full linearization
\begin{align}
    \out_x&=\mathcal{T}^2_{x''}W^2\mathcal{T}^1_{x'}W^1x+\mathcal{T}^2_{x''}(W^2\mathcal{T}^1_{x'}b^1+b^2)\\
    &:=\textbf{W}^{MLP}_x x+\textbf{b}^{MLP}_x
\end{align}
The final output is thus
\begin{align}
    \out_x &= \textbf{W}^{MLP}_x \textbf{W}_x x+\textbf{W}^{MLP}_x\textbf{b}_x+\textbf{b}^{MLP}_x\\
          &:=\Gamma_x x + \gamma_x
\end{align}

As a result, one can see $\textbf{W}_x$ as the CNN induced template that will be mapped on $x$, $b_x$ the induced bias which are not yet class dependant but input dependant, and finally $\Gamma_{x}(y)$ as the induced class induced template for input $x$ and class $y$.



We will now use the above formulation to analyze the behavior and actual computation of the network in the next section.


% we already have this in section 2
\begin{comment}
\begin{figure}[t!]
    \centering
    \includegraphics[width=5in]{Figs/image_x.jpg}
    \caption{Standard way of reshaping an multi-channel input into a column vector in order to perform the convolution and other operations through product matrix-vector.Reshaping of $x$.}
    \label{x_reshaping}
\end{figure}
\end{comment}


\randall{here we have equality $f(\bx_0|\bx_0) ~=~ A \bx_0 + \bd$ as the conditioning is the same as the used point}
\richb{why can't we also have this for $\bx \approx \bx_0$ like above?}\randall{We can but then it is not $=$}
where 
\begin{align}
A =
\label{eq:linearA}
\end{align}
and 
\begin{align}
\bd = 
\label{eq:lineard}
\end{align}


Compare/contrast to taking derivative of $f$ to get $A$ (cannot get $\bd$ that way - why is this a big deal?).
\randall{people already tried to look at what part of the input was used by taking derivative of the output w.r.t to the input leading to finding $A^T$ yet without the bias term which is important as it is not constant but actually containes all the used templates too and thus are part of the representation of the input.}


That is, while a CNN is highly nonlinear function, when conditioned on the input signal $x$, the output function $v$ is a straightforward linear/affine function of the input \dots 
This is concordant with the optimal strategy for classification discussed in the Introduction.

\fi



\iffalse
\subsection{Elastic Map}
Interestingly, the presented analysis of deep networks allow for a natural reformulation via elastic map models. We first present briefly what is elastic map and then highlight how a deep neural network can be seen as such a model allowing a new general approach to current tasks.
\subsubsection{Elastic Map}
An elastic map is a collection of nodes we denote by $W_{i}\in \Omega$ where $\Omega$ is the space of the input data which is usually $\mathbb{R}^D$ we have $K$ such nodes.
Each datapoint of a given and finite training set $x_n\in X$ where $X$ corresponds to the collection of training samples, is paired with the closest node $W_{i}$. Since each datapoint is allocated to only one node, the allocation scheme creates a partition of $X$ into $K$ subsets defined as
\begin{equation}
    X_k=\{x \in X | k=\min_{i=1,\dots,K} d(x,W_i)\},
\end{equation}
which can be seen as a k-NN partitioning of the space. Given this, an energy function $D$ is derived as 
\begin{equation}
    D = \frac{1}{2}\sum_{k=1}^K\sum_{x \in X_k} ||x-W_k||^{2},
\end{equation}
which again can be interpreted as a k-mean loss.

However,  two additional penalty terms are derived : the stretching energy $U_E$ and the bending energy $U_G$,
\begin{equation}
    {\displaystyle U_{E}={\frac {1}{2}}\lambda \sum _{(W_{i},W_{j})\in E}\|W_{i}-W_{j}\|^{2}}
\end{equation}
The bending energy is 

\begin{equation}
    {\displaystyle U_{G}={\frac {1}{2}}\mu \sum _{(W_{i},W_{j},W_{l})\in G}\|W_{i}-2W_{j}+W_{l}\|^{2}}
\end{equation}
        
The total energy of the elastic map is thus 
\begin{equation}
    U=D+U_{E}+U_{G}.
\end{equation}
\subsubsection{Deep Elastic Map}
Interestingly, the presented nodes $W_i$ can be thought as the induced templates from the deep neural network. It is clear that at a given step, there will be at most as many observed templates as there are of training points and we defined them with the same notations as before.
\fi
\iffalse
\subsection{Batch size and weight initialization}\label{section_batch}

\subsubsection{Weight Initialization: Avoiding Sparsity}
As it has been studied for examples in \cite{keskar2016large} the effect of batch size impacts final performances. As a matter of fact, it seems to be as crucial as the impact of weight initialization studied in \cite{glorot2010understanding} and \cite{he2015delving} for the ReLU.
With the proposed framework we will now see first that a random initialization which does not allow enough path to be activated during the first stage of the training is detrimental as neurons can not specialize effectively. Also we will that a too small batch size leads to no convergence as the activated path try to perfectly match the input and this for each input which are different for each batch whereas a too large batch size leads to an averaging of all the activated path for the images in the batch leading to a vague objective.
\begin{figure}[t!]
    \centering
    \includegraphics[width=5in]{Figs/reconstruction_init_linear.jpg}
    \caption{Reconstruction of MNIST images with a deep but linear model w.r.t. different initialization schemes for the filter weights.}
    \label{reconstruction_init_linear}
\end{figure}
In Fig. \ref{reconstruction_init_linear} the initialization is studied for the case of a deep linear model as the one presented in the first section. It is interesting to see that  the normal initialization is very sensitive to the used standard deviation. In fact, for the case of the HeNormal, results are satisfactory whereas for a standard normal distribution they are not. This is justified by the fact that with a very small standard deviation, no outliers are present and thus not filters are advantaged compared to others. However we can see that the uniform initialization is much more robust to this change since the range of the distribution is more likely to be spread on all filters by definition. Note that this effect becomes stronger as the size of the filters decreases. 
\begin{figure}[t!]
    \centering
    \includegraphics[width=5in]{Figs/reconstruction_init_nonlinear.jpg}
    \caption{Reconstruction of MNIST images with a deep but nonlinear model w.r.t. different initialization schemes for the filter weights.}
    \label{reconstruction_init_nonlinear}
\end{figure}
In Fig. \ref{reconstruction_init_nonlinear} is the more realistic case of a deep nonlinear CNN. In this case, and due to the ReLU nonlinearity as well as the max-pooling, the uniform distribution looses its strength when with a $0$ mean. In fact, the artifacts appearing simply translate the fact that random filters are turned off due to their negative output w.r.t. the input. This effect is also present for the normal distribution and the orthogonal one.
We also present in Tables \ref{table_init1},\ref{table_init2} the mean squared error for each policy.
\begin{table}
  \centering
\begin{tabular}{|c|c|} \hline
     &  Deep Linear  \\ \hline
GlorotUniform     &$ 6515.91 \pm 5696.98 $ \\ \hline
HeUniform        & $ 1855.46 \pm 1652.13 $\\ \hline
Orthogonal       & $ 4603.34 \pm 4037.88 $\\ \hline
Constant(1)      & $ 1.16928e+17 \pm 9.57835e+16$\\ \hline
GlorotNormal     & $ 5970.26 \pm 5221.98$\\ \hline
HeNormal         & $ 1199.33 \pm 1064.83$\\ \hline
Normal (0.01,0.005) &$ 0.13544 \pm 0.121944 $ \\ \hline
Uniform(0,0.02) &$ 0.13641 \pm 0.122842$\\ \hline
Normal &$ 0.0989197 \pm 0.0885924$\\ \hline
Uniform  &$0.0985503 \pm 0.0882472$\\ \hline
\end{tabular}
\caption{Mean Squared Error for different initialization schemes for a deep linear model.}
\label{table_init1}
\end{table}
\begin{table}
  \centering
\begin{tabular}{|c|c|} \hline
     &  Deep NonLinear  \\ \hline
GlorotUniform     & $6881.86 \pm 6015.32$  \\ \hline
HeUniform        &  $5240.78 \pm 4559.6$\\ \hline
Orthogonal       &  $5775.77 \pm 5034.57$\\ \hline
Constant(1)      &  $ 2.66836e+17 \pm 2.25564e+17$\\ \hline
GlorotNormal     &  $6547.85 \pm 5710.68$\\ \hline
HeNormal         &  $ 2974.59 \pm 2574.3$\\ \hline
Normal (0.01,0.005) &$0.147991 \pm 0.133734$ \\ \hline
Uniform(0,0.02) & $0.146517 \pm 0.132386$\\ \hline
Normal & $0.0988055 \pm 0.0884875$\\ \hline
Uniform  &$ 0.0982822 \pm 0.0880011$\\ \hline
\end{tabular}
\caption{Mean Squared Error for different initialization schemes for a deep nonlinear model.}
\label{table_init2}
\end{table}
Note that all the experiments are done on MNIST which have mean $0$ and infinite norm to $1$.


The first initialization will determine which paths are active for which inputs and classes on a few batches before the learning made the filters specialize enough to not allow greater changes in the structure. By definition and as it has been discussed in \cite{srivastava2014understanding}, if some paths are never reached quickly they will forever disappear since they can not compete with the optimized paths even though some tricks s.a.  stochastic pooling and dropout can allow recovery. Yet, it is clear that early stage of training is crucial.
We thus see that a good policy to initialize weights is to avoid sparsity in the distribution as is the case for the Normal distribution. In fact, this assumes and induces sparsity in all the activations maps throughout the network yet with random initialization the average energy per feature map is diluted everywhere as a random filter when applied to a structured inputs will not have a bimodal distribution but uniform \cite{henaff2014local}. As a result, having uniform filters in the inner layer will allow for an equitable consideration of all the features at all position instead of being just the ones lucky enough to be initialized with a great enough value. This effect translates directly in the presented figure as being with the wrong assumption on the activations map leading to bad reconstruction from the beginning. This will allow the network to specialize the filters according to what will provide the best gain instead of optimizing on a small range of parameters due to the sparser activations.

\subsubsection{Batch Size: Need for Dynamic Policy}

Now the effect of batch size is different. Having a batch size of $1$ means that whatever path is active the gradient descent update will try to match the input exactly and thus doing this for all input will never lead convergence unless there is one active path per example of some similar examples for part of the path. Now with a large batch size, multiple examples will share the paths especially at the beginning of the learning where no weights are learned. We refer to the paper of \cite{keskar2016large}.


As a matter of fact, with random initialization whatever scheme was used and even though the Danielson Lanczos Theorem applies, the paths are still fairly random. As a result if in the batch there is only one or a few examples per paths, then one ends up trying to minimize 
\begin{equation}
    \mathcal{L}=-\log(\Gamma_{x_1,y_1}x_1)-\log(\Gamma_{x_2,y_1}x_2),
\end{equation}
which can be easily solved by the huge amount of degrees of freedom and the fact that they are not the same of each of the input thanks to the different activation paths. Now if ones uses a large batch, then multiple examples and possibly multiple examples of the same class will have a large part of their path which is common making the network learning in the wrong direction right away by trying to jointly optimize similar degrees of freedom. As a result, we can see that one tremendous strength of artificial neural networks and CNNs in particular is the fact that the path is only a subset of the parameters and only on these the optimization takes places for each example. This is also one way to see that advantages of activation functions with an effective domain where it has value of $0$ as opposed to hyperbolic tangent for example.

\begin{figure}[t!]
    \centering
    \includegraphics[width=5in]{Figs/experiment_batch_size.jpg}
    \caption{Accuracy on MNIST for different batch sizes and the proposed adaptive batch size starting with a really small batch yet increasing the size gradually in dark green. We see that small batch sizes are better yet unstable, this scheduled increases resolves this problem.}
    \label{batch_size}
\end{figure}


This is seen in Fig. \ref{batch_size} where one can also see that even though a small batch is advantageous early, increasing the batch size progressively help to generalize by learning more globally. This is not a problem anymore since the global path are still the best path since learned before thus two similar activated path can only result from close input and not just randomness.







\subsection{The trick -- this text has NOT USED (YET) but can move up}

Assume ReLU and Max Pooling.
Max Pooling is a ``keep or kill'' transformation.
ReLU, since it is soft thresholding \randall{in this paper we do not show the link between ReLU and soft threshlolding explicitly but we will in the next} is nearly ``keep or kill.''
This means that, if an activation map pixel advances from one layer to the next, then its value is basically unchanged.
Also, we can trace back from any nonzero value at the output of the entire network all the way to the input; this ``track'' has nonzero values through all layers.
The track is actually a tree that can branch out to have more branches as we move back towards the input.
There will also be tracks that start at the input but that are suppressed by ReLU or Max Pooling at an intermediate level of the network; these paths have no effect on the value of the output.
This has already been discovered by LeCun et al \cite{X}; anyone else?
\randall{actually it is done during the forward pass, the activation indices of max pooling and relu are kept in memory and also needed for back propagation}

This lets us write a formula for the output of the network given an input image $x$.
\bigskip

\centerline{\bf then a miracle occurs}

Theorem:  Given an training input data pair $(x_i, y_i=q)$ (i.e., from class $q$), the output vector $v(m)$ of a CNN (suitably trained, etc.) approximates a matched filter bank (as introduced in the intro):
%
\begin{align}
v(m) ~=~ \langle x, \tau_m \rangle
\end{align}
%
where $\tau_q \approx x$ and $\tau_m \perp \tau_q, m\neq q$\randall{this is the optimal, not necessarily what actually happens though}.

In words, the CNN learns to compute a GLRT type classifier from training data, which is optimal.  
Of course this is just for the training data.

Segue into the other concepts:

This explains memorization, etc. etc.

\subsection{Remarks (basically the rest of the paper)}

These need to be built out into subsections/theorems.

R1: The CNN learns a {\em large set of templates} to represent signals with only one (best basis in term of sparsity/entropy), the number of templates is literally the number of possible paths in the activation graphs plus modulations on the amplitudes thus infinite.
The CNN tries to disentangle independent features to represent all images and the MLP part does the classification as it could be with a kernel SVM.


The first layer forms the basic atoms (overcomplete basis of training set size or larger) and later layers form combinations of those atoms to form templates. Every template is a linear combination of the first layer atoms but then the inner layers define how they should behave together, in a sense deeper layer shape the possible distributions of those atoms to form an actual images and not random edges everywhere (also true for GAN).
This is (\ref{eq:z|x}).  \richb{how large}




R3: Moreover, the representation of $x$ (by the AT) is the {\em optimal} set of atoms in the dictionary.  
That is, while finding the best set of atoms from the dictionary is combinatorially complex, the CNN performs an iterative, local (greedy) optimization that finds the global optimum.
This is Section \ref{sec:pullmax} below.
Analog to ``best basis'' algorithms a la my paper, donoho paper, coifman paper.

R4: We can understand a lot from this viewpoint, including adversarial examples, which are designed to perturb (\ref{eq:condOutput}), memorization, ...
This is a large part of the rest of the paper.

R5: GAN comment:  Since we show memorization is easy for NNs, the discriminator is always better unless the generator replicates exactly the training set otherwise the discriminator can always adapt and this is coherent with the ICLR talks on GAN.  
In short, GANs are imply a machine learning to map random noise to one of the training set examples, it is good to see that people finally realize GANs are simply copying the dataset ! 
\fi

==> richb.tex <==
\section*{RichB thoughts}

\begin{enumerate}

    \item This is {\em super cool!}
   
   \item Does this explain why CNNs work with occlusion?  (Can turn off 1/2 of a template)
   
   They work well as long as the template matching captures most of the energy and the occlusion has low energy, but yes, the local sub-templates activations can be enough to let the neuron fires telling that the object is still present.
 
    \item Relation to Donoho/Wakin manifold projection?
    
    I think the most straightfoward is the fact that lower layer encode details whereas higher tries to have the global scheme whatever was the details or their possible diffeomorphisms which is why a template is not just a combination of sub templates but actually also a combination of the possible deformations of the sub templates. I think then that a training scheme a la Donoho/Wakin could be to train the upper layer on smoothed image $x\star \mathcal{N}_2$ then use this layer as the upper one and add a new layer below and train the 2 layer net on a less smooth version of the image $x\star \mathcal{N}_1$ and so on till all the layers are present and trained on the raw image. But we have to investigate more oon this idea.
    
    \item What's the
``template manifold'' 
that can be reached by this approach?  What are its properties?

With this approach, basically I think that with the right weighting of all the templates and sub-templates one can generate almost all images, a bit like random filters can recreate arbitrary signals with the right weighting. Now the idea is as follows, as we stop weighting the low level sub-templates, we will see in the image the complete template appearing without weighting of the sub-templates and thus we loose precision and win in term of matching the input with its closest full template. This also explains why the last paper on improved GAN (\url{https://arxiv.org/pdf/1612.00005v1.pdf}) is very good because now they constrain not just the last layer weighting as in standard GAN but all the sub weighting too !

\item Mauro Maggioni ``manifold wavelet'' stuff could be relevant for the template manifold

ahah indeed I am actually looking into diffusion wavelet with a friend in Paris, there are indeed many connections with CNN and scattering. I think this would mainly be "high level" correspondences though.
    
\item What does this say about generalization of CNNs?  Does it help address Ben Recht's concerns in his new paper?

Basically, what's shown in this paper is that the modeling capability of CNN is like decision tree, they can in fact learn the dataset whatever the labels. This is quite reasonable to think about since by definition on the training set it is sufficient to learn templates that are somehow a sum of the images of the same class (to simplify) and thus the template matching would still lead to 0 error on the training set.
    
\end{enumerate}


main points :
\begin{itemize}
    \item CNN can be built from a template matching POV with robustness to deformations : GOOD
    \item CNN can only max out local translation perturbations, everything else has to be sum out -> ADVERSARIAL EXAMPLE
    \item CNN by the factorization can only learn wavelet like filters or combination of wavelets based on the activation correlations.
    \item Any ANN learned on a deterministic dataset achieves 0\% training error even with random labels
    \item we can now explain almost everything from activation functions to models
    \item WE PROPOSE : 
    \begin{itemize}
        \item introduce max over channels for max out of other kind of transforms (robust to adversarial)
        \item introduce per layer diffeomorphisms and max out and activation miniloss (no over fitting anymore)
        \item introduce skip connections and different filter sizes from long range correlation learning (represent anything clean)
        
    \end{itemize}
\end{itemize}
the CNN part tries simply to find the best possible adapted template given its filters and templates. Once found $phi_x$ the output of the CNN is fed into a perceptron which is the one making the decision process (the CNN always tries to match everything even filters that would not be needed for the present input class) so this final layer then does the actual matching between its weights associated with the class to predict and its input (output of the CNN).
So we have to think about what is the best, to say that a template matching is done between the CNN and classifier (perceptron) or between those two and the input ?
Because after all the CNN simply does a complex nonlinear change of basis that's all, the real test is done by the perceptron.

it turns out that our big matched template is actually after all the computation exactly the jacobian of the output w.r.t the input image !
Basically now we have exactly that the output of big personalized template $phi_{x,k}$
is $<phi_{x,k},x>$ which is now equal to $<df_{k,x}/dx,x>$ where I didn't put many notations but $f_{k,x}$ is the network on the $k^th$ output template and conditioned on $x$. Thus for all output neurons means that basically we compute simple distances with some local planes where those planes are input dependent (adaptive to the input).






is $<phi_{x,k},x>$ which is now equal to $<df_{k,x}/dx,x>$ where I didn't put many notations but $f_{k,x}$ is the network on the $k^th$ output template and conditioned on x. Thus for all output neurons means that basically we compute simple distances with some local planes where those planes are input dependent (adaptive to the input).


This also explains adversarial example very easily actually since
the new image is $x+df_{x,k}/dx$ where $x$ is from class j, then after application we have for template j and k respectively

\[
<x+df_{x,k}/dx,Phi_{x,j}>,<x+df_{x,k}/dx,Phi_{x,k}>
\]
which is now equal to
\[
<x+df_{x,k}/dx,df_{x,j}/dx>,<x+df_{x,k}/dx,df_{x,k}/dx>
\]
which is respectively
\[
<x,df_{x,j}/dx>+<df_{x,k}/dx,df_{x,j}/dx>,<x,df_{x,k}/dx>+||df_{x,k}/dx||^2
\]
so as soon as the two adv. classes have template a bit uncorrelated $<df_{x,k}/dx,df_{x,j}/dx>$ is small and by definition $<x,df_{x,k}/dx>$ should be as small so we end up comparing
$<x,df_{x,j}/dx>$ and $||df_{x,k}/dx||^2$ where by definition  the latter is bigger unless the input image is a perfect fit with the induced template.

